End-to-End Balancing for Causal Continuous Treatment-Effect Estimation

We study the problem of observational causal inference with continuous treatments in the framework of inverse propensity-score weighting. To obtain stable weights, we design a new algorithm based on entropy balancing that learns weights to directly maximize causal inference accuracy using end-to-end optimization. In the process of optimization, these weights are automatically tuned to the specific dataset and causal inference algorithm being used. We provide a theoretical analysis demonstrating consistency of our approach. Using synthetic and real-world data, we show that our algorithm estimates causal effect more accurately than baseline entropy balancing.

==> check.tex <==
\begin{onehalfspacing} 

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{We have outlined the key assumptions in the Problem Definition section and discussed the potential impact of their violation in the Broader Impact section.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See the Broader Impact and Limitations section.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{in the Problem Definition and Analysis sections.}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{see Appendix \ref{sec:proofs}}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNo{The code and the data are proprietary. However, we provide the instructions in the experiments section and the details in Appendix \ref{sec:details}.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{we provide the instructions in the experiments section and the details in Appendix \ref{sec:details}.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See the Broader Impact section.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{See \citep{Rappold2020}.}
  \item Did you mention the license of the assets?
    \answerYes{It is U.S. Public Domain License.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

\end{onehalfspacing}
\linespread{1}  
\newpage
\clearpage

==> extra.tex <==


\subsection{The Derivative}
\label{sec:deriv}

\begin{align*}
    &\sum_{i=1}^{n}\bm{g_i}\exp\left( \bm{g}_i^{\top}\bm{\lambda}^{\star}+\ell_i\right) = \bm{0}\\
    &\frac{\partial}{\partial \ell_i} \left\{\sum_{i=1}^{n}\bm{g_i}\exp\left( \bm{g}_i^{\top}\bm{\lambda}^{\star}+\ell_i\right) \right\} = \bm{g}_i\exp\left( \bm{g}_i^{\top}\bm{\lambda}^{\star}+\ell_i\right) +  \left\{\sum_{i=1}^{n}\bm{g}_i\bm{g}_i^{\top}\exp\left( \bm{g}_i^{\top}\bm{\lambda}^{\star}+\ell_i\right) \right\}\frac{\partial \bm{\lambda}^{\star}}{\partial \ell_i}
    % &\frac{\partial}{\partial \bm{\lambda}} \left\{\sum_{i=1}^{n}\bm{g}_i\exp\left( \bm{g}_i^{\top}\bm{\lambda}^{\star}+\ell_i\right) \right\} = \sum_{i=1}^{n}\left\{\bm{g}_i\bm{g}_i^{\top}\exp\left( \bm{g}_i^{\top}\bm{\lambda}^{\star}+\ell_i\right) + \bm{g}_i\exp\left( \bm{g}_i^{\top}\bm{\lambda}^{\star}+\ell_i\right) \frac{\partial \ell_i}{\partial \bm{\lambda}} \right\}= \bm{0}\\
    % &\sum_{i=1}^{n}\bm{g}_i\bm{g}_i^{\top}\exp\left( \bm{g}_i^{\top}\bm{\lambda}^{\star}+\ell_i\right) + \sum_{i=1}^{n}\bm{g}_i\exp\left( \bm{g}_i^{\top}\bm{\lambda}^{\star}+\ell_i\right) \frac{\partial \ell_i}{\partial \bm{\lambda}} = \bm{0}
\end{align*}

